Some connections between universal algebra and logics for trees

One of the major open problems in automata and logic is the following: is there an algorithm which inputs a regular tree language and decides if the language can be defined in first-order logic? The goal of this paper is to present this problem and similar ones using the language of universal algebra, highlighting potential connections to the structural theory of finite algebras, including Tame Congruence Theory.

==> booldet.tex <==
\section{Path Languages}
In this section we try to give an effective characterization of path languages. Recall that, by Lemma~\ref{lem:path-algebra-path-clone}, path languages are the same thing as Boolean combinations of languages recognised by deterministic top-down tree automata, and are also the same thing as languages recognised by matrix powers of the two-element lattice.


\subsection{Separation} We say that two tree languages can be \emph{separated by a deterministic top-down automaton} if there is a deterministic top-down tree automaton which accepts all trees in one of the languages, and rejects all trees in the other language.

Consider a finite algebra $\alg$. Define an $n$-port tree over $\alg$ to  be a tree where internal nodes are labelled by operations of the algebra (of arity at least one), and where leaves are labelled by elements of the universe or by variables in the set $\set{x_1,\ldots,x_n}$.  To each $n$-port tree corresponds an $n$-ary polynomial, but different $n$-port trees might yield the same polynomial. We write $\treesar n \alg$ for the set of $n$-port trees over $\alg$. A \emph{tree over $\alg$} is the special case of a $0$-port tree over $\alg$, its value is the corresponding $0$-ary polynomial, i.e.~element of $\alg$.  


When $\alg$ has finitely many operations, then $\trees \alg$ is a set of trees over a finite ranked alphabet. Therefore, one can run automata on trees from $\trees \alg$. 

\paragraph*{Mixes.} For a tree $t$ over a ranked alphabet $\Sigma$, and a root-to-leaf path $\pi$ in $t$, define $t|\pi$ to be the word which indicates the labels and directions taken by the path $\pi$, as depicted in the following picture:
\begin{center}
	(TODO picture)
\end{center}
For a set $L$ of trees over a ranked alphabet $\Sigma$, a tree $t$ is called a \emph{path mix of $L$} if  for every root-to-leaf path $\pi$ in $t$, there exists a tree $s \in L$ and a root-to-leaf path $\sigma$ in $s$ such that  $t|\pi = s|\sigma$. The following lemma is folklore.

\begin{lemma}\label{lem:mixes}
	If $L$ is a tree language recognised by a finite algebra, then also the set of path mixes is recognised by a finite algebra, which can be computed based on the algebra recognising $L$.  Furthermore, the set of path mixes is the least, with respect to inclusion,  deterministic language that contains  $L$.
\end{lemma}

For a finite algebra $\alg$, and a subset $B$ of its universe, let us define $\mix_\alg B$ to be the set of elements $a \in \alg$ such that there is some tree $t \in \trees \alg$ which has type $a$, and which is a mix of trees which have types in $B$.  A corollary of Lemma~\ref{lem:mixes} is that $a_0,a_1$ in $\alg$ can be separated by a deterministic language if and only if $a_0 \not \in \mix_\alg \set{a_1}$ or $a_1 \not \in \mix_\alg \set {a_0}$. Furthermore, this condition can be effectively checked.

%
%
% $\pathset \alg$ to be the set of words
%
% For a signature $\Sigma$, define $\pathset \Sigma$ to be the set of words which describe paths in trees over $\Sigma$. For $\pi \in \pathset \Sigma$ and $t \in \trees \Sigma$, we
% \begin{lemma}\label{lem:}
% 	One can decide if two regular tree languages can be separated by a determinstic top-down automaton.
% \end{lemma}
% \begin{pr}[Folklore]
% 	If $L \subseteq \trees \Sigma$ is regular, then
% 	\begin{align*}
% 		\pathset L \eqdef \set{}
% 	\end{align*}
% \end{pr}
\paragraph*{Separating $\lor$-pairs.}
An \emph{$\lor$-pair} in an algebra $\alg$ is a pair $a_0,a_1$ of elements in the universe on which  some  $f \in \polar 2 \alg$ acts like $\lor$, i.e.~
	\begin{align*}
		(\set{a_0,a_1},f) \simeq (\set{0,1}, \lor).
	\end{align*}
	A $\land$-pair is defined dually.


\begin{lemma}\label{lem:no-mix}
	In a path algebra, every $\lor$-pair can be separated by a deterministic top-down automaton.
\end{lemma}


\subsection{Types of a minimal non-trivial congruence}
A pair $(\alpha,\beta)$ of congruences in a finite algebra $\alg$ is called \emph{prime} if $\alpha$ is finer than $\beta$, and there is no other congruence between them. 
The book HM shows, in Definition 5.1, how to assign to each prime pair of congruences (actually a slightly more general notion of tame pair is used) a type, which is a number in $\set{1,\ldots,5}$. We will be interested in prime pairs of the form $(0_\alg,\alpha)$, where $0_\alg$ is the identity congruence and $\alpha$ is a non-identity congruence that is minimal (with respect to inclusion, when a congruence is seen as a binary relation).

We say that an algebra $\balg$ divides an algebra $\alg$ if $\balg$ can be obtained from $\alg$ by first removing operations, then restricting the universe, and then taking a quotient under a congruence.
\begin{lemma}\label{lem:one-or-five}
	Let $\alpha$ be a minimal non-trivial congruence in a finite algebra $\alg$. If $\alg$ is a path algebra, then  $(0_\alg,\alpha)$ has type 1 or  5.
\end{lemma}
\begin{pr}
	We use the following properties of types: 
	\begin{itemize}
		\item if some prime pair of congruences in $\alg$ has type 2, then $\alg$ is divided by a group algebra, i.e.~an algebra where the universe is a finite group, and there is a binary operation for the group operation;
		\item if some prime pair of congruences in $\alg$ has type 3, then $\alg$ is divided by the two-element Boolean algebra $(\set{0,1}, \lor, \neg)$;
				\item If some prime pair of congruences in $\alg$ has type 4, then $\alg$ is divided by the two-element lattice  $(\set{0,1}, \lor, \land)$.
	\end{itemize}
	Since path algebras are closed under division, and all of the divisors described in the above items are not path algebras, it follows that a path algebra cannot have a prime pair of congruences of types 2,3 or 4.
\end{pr}
\subsection{Type 5 congruence}


\begin{lemma}\label{lem:}
	Let $\alpha$ be a minimal non-trivial congruence in a finite algebra $\alg$ such that  $(0_\alg,\alpha)$ has type 5. Then $\alg$ is a path algebra if and only if:
	\begin{enumerate}
		\item $\alg/_\alpha$ is a path algebra; and
		\item every $\lor$-pair can be separated by a deterministic top-down automaton.
	\end{enumerate}
\end{lemma}
\begin{pr}
	The only if implication follows from Lemma~\ref{lem:no-mix} and closure of path algebras under congruence quotients. Let us then do the ``if'' implication, i.e.~suppose that items 1 and 2 in the lemma hold. We use the following claim which follows from Hobby and McKenzie
	
	\begin{claim}
		If $a,b$ be distinct elements in the universe of $\alg$ which are equivalent with respect to $\alpha$, then there is some $f \in \polar 1 \alg$ such that $f(a),f(b)$ is a $\lor$-pair or $\land$-pair.
	\end{claim} 
	\begin{pr}[Check]
		 Hobby and McKenzie  show in Theorem 2.8 item (4), that there is some $f \in \polar 1 \alg$ which maps the whole universe to a minimal set  $f(A) \in M_\alg(0_\alg,\alpha)$, and  such that $f(a) \neq f(b)$. As far as I understand the definition of traces, namely Definition 2.15,  $f(a)$ and $f(b)$ are in a single $(0_\alg,\alpha)$-trace. Finally, Lemma 4.15 items (1) and (2) imply that every $(0_\alg,\alpha)$-trace has exactly two elements, which form a $\lor$-pair or $\land$-pair depending on the order in which they are given.
	\end{pr}
	
Let then $a,b$ be as in the claim.	By condition 2, there is a deterministic language $L$ which contains all trees that evaluate to $f(a)$, and which is disjoint with all trees that evaluate to $f(b)$. The language $f^{-1}(L)$ is also deterministic, and it separates $a$ from $b$. In other words, the claim implies that every two distinct $\alpha$-equivalent elements $a,b$ of the universe are separated by  a top down deterministic automaton $\alg_{ab}$. It follows $\alg$ divides  the product of these automata together with the path automaton for $\alg/_\alpha$.
\end{pr}


\subsection{Type 1 Congruence}

A congruence $\alpha$ in an algebra $\alg$ is called \emph{strongly abelian} if  for every $n \in \Nat$ and every $f \in \polar n \alg$, the implication
\begin{align*}
	f(a_0,\ldots,a_n) = f(b_0,\ldots,b_n) \qquad \mbox{implies} \qquad f(a_0,c_1,\ldots,c_n)=f(b_0,c_1,\ldots,c_n)
\end{align*}
holds for every $a_0,\ldots,a_n, b_0,\ldots,b_n, c_0,\ldots,c_n$ in the universe of $\alg$ such that $a_i,b_i,c_i$ are all $\alpha$-equivalent for every $i \in \set{0,\ldots,n}$. Theorem 5.6 of HM says that  if $\alpha$ is such that $(0_\alg,\alpha)$ has type 1, then $\alpha$ is strongly abelian.  The missing part in our proof is a lemma of the following form:
\begin{lemma}\label{lem:}
	Let $\alpha$ be a minimal non-trivial congruence in a finite algebra $\alg$ such that  $(0_\alg,\alpha)$ has type 1 (and therefore $\alpha$ is strongly abelian). Then $\alg$ is a path algebra if and only if
	\begin{enumerate}
		\item $\alg/_\alpha$ is a path algebra; and
		\item (some condition that is not known yet)
	\end{enumerate}
\end{lemma}

% A regular word colouring is a function from words over a finite alphabet to a finite set of colours, such that for every colour, its inverse image under the colouring is a regular language of words.
% \begin{lemma}\label{lem:}
% 	Suppose that $\alg$ is a path $\Sigma$-algebra. There exists a regular colouring
% 	\begin{align*}
% 		\lambda : \pathset \Sigma \to C
% 	\end{align*}
% 	and a number $m \in \Nat$ with the following property. Let $a \in A$ and $B \subseteq A$ be such that $a \in \mix B$. Then  for every $p \in \pol_m \Sigma$ where
% \end{lemma}




==> conclusion.tex <==
\section{Conclusion}
We discussed the following logics for trees:
\begin{enumerate}
	\item chain logic, i.e.~\mso with set quantification restricted to chains;
	\item path languages, i.e.~Boolean combinations of deterministic top-down tree automata;
	\item a variant of {\sc ctl}.
	\item first-order logic with descendant and child relations;
\end{enumerate}
In the first three cases but not in the last one,  the definability problem is equivalent to checking if  the syntactic algebra belongs to a class of finite algebras closed under  polynomial equivalence. Furthermore, the first three logics can be characterised in terms of the following algebra classes discussed in~\cite{vanderfwerf}: (1) is matrix powers of wreath products of $(2,\land)$; (2) is matrix powers of $(2,\land)$; (3) is wreath products of $(2,\land)$. 

==> smieci.tex <==

 satisfies conditions (LQ) and (LB) in Lemma~\ref{lem:clone-invariant}, but fails condition (LH), about inverse images of clone morhpisms. The issue is that a clone morhpism can duplicate trees. For instance, let $f_0,f_1,f_2$ be letters as in the previous example, of arities $0,1,2$ respectively. Consider the signatures $\Sigma = \set{f_0,f_2}$ and $\Gamma=\set{f_0,f_1}$. As discussed in the previous example, the set of trees where every leaf is at even depth is first-order definable when the signature is $\Sigma$, but is not first-order definable when the signature is $\Gamma$ (note that in the latter case every tree has just one leaf).  Consider the morphism 
\begin{align*}
	\alpha : \clo \Gamma \to \clo \Sigma
\end{align*}
which maps $f_0$ to $f_0$, and which maps $f_1(t)$ to $f_2(\alpha(t),\alpha(t))$. This morphism maps a tree that looks like a line to a complete binary tree of the same depth. The set of trees over $\Gamma$ which have the unique leaf at even depth is the inverse image under $\alpha$ of the set of trees over $\Gamma$ which have every at even depth. One can show that the first-order definable tree languages satisfy a weak condition than (LH), where morphisms are restricted to nonduplicating ones, i.e.~morphisms $\alpha$ where a tree $a(t_1,\ldots,t_n)$ is mapped to a term which uses each of  $\alpha(t_1),\ldots,\alpha(t_n)$ at most once.


\begin{defi}
Define a \emph{polynomial pseudovariety} to be an isomorphism closed  class $\mathscr V$ of finite algebras, which is closed under: 
\begin{enumerate}
	\item {\bf reducts:} if $\aalg \in \mathscr V$, then every reduct of $\aalg$ is also in $\mathscr V$.
	\item {\bf subalgebras:} if $\aalg \in \mathscr V$, then every subalgebra of $\aalg$ is also in $\mathscr V$.
	\item {\bf products:} if $\aalg,\balg \in \mathscr V$, then $\aalg \times \balg \in \mathscr V$.
	\item {\bf quotients:} if $\aalg,\balg \in \mathscr V$ and $\sim$ is a congruence of $\aalg$,  then $\aalg/_\sim \in  \mathscr V$.
	\item {\bf polynomial equivalence:} if $\aalg \in \mathscr V$, then every finite algebra polynomially equivalent to $\aalg$ is also in $\mathscr V$.
\end{enumerate}
\end{defi}



\begin{thm}
Let $\mathscr L$ be a class of regular tree languages satisfying:
\begin{itemize}
		\item[(LQ)] If $\mathscr L$ contains a tree language  $L \subseteq \trees \Sigma$ then $\mathscr L$ also contains 
		\begin{align*}
			p^{-1}L = \set{t \in \trees \Sigma : pt \in L} \qquad \mbox{ for every $p \in \polar 1 \Sigma$.}
		\end{align*}
		\item[(LB)] $\mathscr L$ is closed under Boolean combinations, including complementation;
		\item[(LH)] if $\mathscr L$ contains a tree language  $L \subseteq \trees \Sigma$, $\Gamma$ is a signature, and
		\begin{align*}
			h: \trees \Gamma \to \trees \Sigma
		\end{align*}
		is a tree homomorphism, then $\mathscr L$ also contains $h^{-1}(L)$.
	\end{itemize}
Then the following class class of finite algebras is a polynomial pseudovariety
\begin{align*}
\mathscr V =  \set{\aalg : \mbox{$\aalg$ is a finite algebra which recognises only languages from $\mathscr L$}}
\end{align*}
Furthermore,  a language belongs to $\mathscr L$ if and only if its syntactic algebra is in $\mathscr V$

\end{thm}

\input{old-clones}
There is by now a wide body of research on the structure of finite algebras. 

Let $\aalg$ be an algebra.  Define a polynomial in $\aalg$ to be a . Define 



\begin{defi}
	A clone consists of:
	\begin{enumerate}
		\item a set $A$, called the \emph{universe of $A$}; and
		\item for every $n \in \set{0,1,2,\ldots}$ a subset $A^n \to A$ which is called the $n$-ary operations in the clone, subject to the following requirements:
		\begin{enumerate}
		\item for every $a \in A$, there is a $0$-ary operation which is the constant $a$;
		\item for every $n \in \set{1,2,\ldots}$ and every $i \in \set{1,\ldots,n}$, the projection
		\begin{align*}
  (a_1,\ldots,a_n) \mapsto a_i
\end{align*}
is one of the $n$-ary operations in the clone;
\item for every $n,k \in \Nat$, if $f$ is an $n$-ary operation in the clone, and $f_1,\ldots,f_n$ are $k$-ary operations in the clone, then the following is also a $k$-ary operation in the clone:
\begin{align*}
  \bar a \in A^k \quad  \mapsto \quad  f(f_1(\bar a),\ldots,f_k(\bar a))
\end{align*}

	\end{enumerate}
		\end{enumerate}
\end{defi}


\begin{align*}
  \pi_{i,n} (c_1,\ldots,c_n)  = c_i
\end{align*}

Define a \emph{clone homomorphism} 
\begin{align*}
  h : \clonec \to \cloned
\end{align*}
to be a function 


The \emph{free clone} over $\Sigma$ is defined to be the following algebraic structure. It has one sort per number $n \in \set{0,1,\ldots}$. The elements of sort $n$ are the $\Sigma$-terms with variables $\set{1,\ldots,n}$. For each $n$ and $n_1,\ldots,n_k$ there is a 


\subparagraph{Clones}
In this paper, we use the name {clone} for what is sometimes referred to as an \emph{abstract clone}. 
Define a clone to be the following algebraic structure. There are  infinitely many sorts $C_0,C_1,\ldots$  indexed by natural numbers. Intuitively speaking  $C_n$ represents  operations which take $n$ inputs and yield one output, and draw them like this:

For every $n,k \in \Nat$ there is a \emph{composition operation}, which takes  $f \in C_n$ and  $f_1,\ldots,f_n \in C_k$, and maps them their \emph{composition} in $C_k$ which is denoted by $f(f_1,\ldots,f_n)$
and drawn like this
\begin{center}
	picture
\end{center}
The composition operation must satisfy the following associativity axiom
\begin{align*}
  (f(f_1,\ldots,f_n))(g_1,\ldots,g_k) = f(f_1(g_1,\ldots,g_k),\ldots,f_n(g_1,\ldots,g_k))
\end{align*}
for every $n,k,l \in \Nat$ and every $f \in C_n$, $f_1,\ldots,f_n \in C_k$ and every $g_1,\ldots,g_k \in C_l$.
Furthermore, for every $n \in \set{1,2,\ldots}$ and every $i \in \set{1,\ldots,n}$ there is a constant $\pi_{i,n}$ which represents the projection and  that satisfies the following axiom:
\begin{align*}
  \pi_{i,n}(f_1,\ldots,f_n) = f_i \qquad \mbox{ for every $k \in \Nat$ and $f_1,\ldots,f_n \in C_k$}
\end{align*}


\subparagraph{The free clone.} Suppose that $\Sigma$ is a ranked set. Define the \emph{free clone over $\Sigma$} to be the clone where $C_n$ consists of $n$-ary terms over $\Sigma$, and the composition operation is term composition defined in the obvious way, as illustrated in the following picture:
\begin{center}
	picture
\end{center}


A \emph{clone} with universe $A$,  is a family of operations  $A^n \to A$, for possibly different arities $n$, which contains all the projection functions $(a_1,\ldots,a_n) \mapsto a_i$ and is closed under composition in the following sense: if $f_1,\ldots,f_k$ are $n$-ary operations in the clone, and $f$ is a $k$-ary operation in the clone, then the clone also contains the following $n$-ary operation
\begin{align*}
	\bar a \mapsto f(f_1(\bar a),\ldots,f_k(\bar a)).
\end{align*}
% A clone can be treated as an infinitely sorted algebra, with one sort for the set $A$, sorts $F_0,F_1,\ldots$ for the  operations, constants for the projection functions, and composition operations
% \begin{align*}
% 	comp_{n,k} : (F_n)^k \times F_k \to F_n
% \end{align*}
If $\Cc$ and $\Dd$ are clones, then a clone morphism 
\begin{align*}
	\alpha : \Cc \to \Dd
\end{align*}
is a function that maps: the universe of  $\Cc$ to the universe of  $\Dd$, and $n$-ary operation in $\Cc$ to $n$-ary operations in $\Dd$, which maps projections to projections and which is consistent with composition.
For an algebra $\Aa$, define its generated \emph{clone}, denoted by $\clo \Aa$, to be the clone where the universe is the same as in $\Aa$, and which has an operation for every term operation in $\Aa$. The \emph{polynomial clone}, denoted by $\pol \Aa$, is defined the same way, except that it has operations for all polynomials in $\Aa$.


If $\Sigma$ is a signature, then we write $\clo \Sigma$ for the clone corresponding generated by the algebra  $\trees \Sigma$, i.e.~for every arity $n$ it has terms with at most $n$-free variables, seen as transformations from $n$-tuples of terms to terms.

%  that respects aritites and is consistent with composition.
% If $\Sigma$, we write $\terms \Sigma$ for the free clone over $\Sigma$. I.e.~for ever $n$, this clone has all terms over $\Sigma$ with $n$ variables
%  is a ranked alphabet and $X$ is a set of variable names, we write
% 	\begin{align*}
% 		\terms {\Sigma,X}
% 	\end{align*}
% 	for the set of terms built using the ranked alphabet $\Sigma$ and variables from $X$. When $X$ is omitted, it is assumed to be empty, i.e.~$\terms \Sigma$ is the set of ground terms. We will view ground terms as trees. For $t \in \terms{\Sigma,X}$, and a valuation $\eta : X \to \terms \Sigma$, we write $t[\eta]$ for the term obtained from $t$ by replacing each variable $x \in X$ by the term $\eta(x)$.
	
	
\paragraph*{Recognising tree languages.} A \emph{tree language} is any subset of $\trees \Sigma$, for some finite signature $\Sigma$.  We say that a function
\begin{align*}
	f : X \to Y 
\end{align*}
\emph{recognises} a subset of $X$ if elements with the same value under $f$ either both belong to the subset,  or both do not belong to the subset. To recognise tree languages, we will use either $\Sigma$-algebra morphisms
\begin{align*}
	\alpha : \trees \Sigma \to \Aa 
\end{align*}
where $\Aa$ is a finite $\Sigma$-algebra, or clone morphisms
\begin{align*}
	\alpha : \clo \Sigma \to \Cc
\end{align*}
where $\Cc$ is a clone. If there is a morphism as in the first case, then we say that the $\Sigma$-algebra $\Aa$ recognises $L$, if there is a morphism as in the second case, then we say that the clone $\Cc$ recognised $L$. Note that a $\Sigma$-algebra can recognise on languages over $\Sigma$, while a clone can recognise languages over various signatures.

It is not difficult to see that a tree language is recognised by a morphism of $\Sigma$-algebras whose target has finite universe if and only if it is recognised by a clone morphism into a clone whose target has finite universe. In either case, the languages is called \emph{regular}.


% Sometimes we are interested in the case when the morphism $\alpha$  has one or both of the following properties:
% \begin{itemize}
% 	\item \emph{letter-to-letter:} letters of $\Sigma$ are mapped to fundamental operations of $\Aa$;
% 	\item \emph{nonduplicating:} nonduplicating terms are mapped to nonduplicating terms.
% \end{itemize}


\paragraph*{Syntactic algebra and clone.} Define the \emph{syntactic congruence} of a language $L \subseteq \trees \Sigma$, also known as $L$-equivalence, to be the relation which considers two trees $s,t \in \trees \Sigma$ equivalent if and only if 
\begin{align*}
	ps \in L \qquad \mbox{iff} \qquad pt \in L \qquad \mbox{holds for every $p \in \polar 1 \Sigma$}.
\end{align*}
In the definition above, we could require that $p$ is non-duplicating, which would give the same notion of syntactic congruence. The \emph{syntactic algebra} of $L$ is the $\Sigma$-algebra obtained by quotienting the free $\Sigma$-algebra $\trees \Sigma$ by the syntactic congruence. The \emph{syntactic clone} is the clone of the syntactic algebra.
	


\paragraph*{Characterising a logic via syntactic clones.} We would like to prove theorems of the form ``a tree language belongs to a class $\mathscr L$ if and only if its syntactic clone belongs to class $\mathscr C$'', preferably with membership in class $\mathscr C$ being decidable. Unfortunately, some classes of languages do not admit such theorems, because the same syntactic clone can be obtained for languages in and outside the class.


\begin{ourexample}\label{ex:potthof} In this example, we show two languages, one first-order definable, and the other not first-order definable, which share the same syntactic clone.
	 Consider a signature $\Sigma$ with letters $f_0,f_1,f_2$, of arities $0,1,2$ respectively.  Let $L \subseteq \trees \Sigma$ be  those trees where every leaf is at even depth.  
	The syntactic $\Sigma$-algebra of this language has three elements, ${0,1,\bot}$, with the functions corresponding to the letters being defined by 
	\begin{align*}
		f_0 = 0 \qquad f_1(a)= \begin{cases}
		0 & \mbox{ if $a=1$}\\
		1 & \mbox{ if $a=0$}\\
		\bot & \mbox{ otherwise}
		\end{cases} \qquad
		f(a,b) = \begin{cases}
			0 & \mbox{ if $a=b=1$}\\
			1 & \mbox{ if $a=b=0$}\\
			\bot & \mbox{ otherwise}
		\end{cases}
	\end{align*}
	The language $L$ is not first-order definable, because a formula of first-order logic cannot distinguish between the trees $f_1^n(f_0)$ and $f_1^{n+1}(f_0)$ for large enough $n$. Define the language $K$ to be the same as $L$, except that the symbol $f_1$ is dropped from the signature. A surprising result by Potthoff~\cite{potthoff} is that the  language $K$ is first-order definable.  The syntactic clone of $L$ is the same as for $K$, because  $f_1$ can be defined by
	\begin{align*}
		f_1(a) = f_2(a,a).
	\end{align*}
\end{ourexample}
 
 
The above example shows that one will not get an effective characterisation of first-order logic on trees just by looking at syntactic clones. Therefore, since this paper is mainly about clones, we will no longer talk about first-order logic. However, as we shall show later on, there are other logics for which the syntactic clone does carry sufficient information.  To prove this, we will use the following lemma.

\begin{lem}\label{lem:clone-invariant} Let $\mathscr L$ be a class of regular tree languages satisfying:
	\begin{itemize}
		\item[(LQ)] If $\mathscr L$ contains a tree language  $L \subseteq \trees \Sigma$ then $\mathscr L$ also contains 
		\begin{align*}
			p^{-1}L = \set{t \in \trees \Sigma : pt \in L} \qquad \mbox{ for every $p \in \polar 1 \Sigma$.}
		\end{align*}
		\item[(LB)] $\mathscr L$ is closed under Boolean combinations;
		\item[(LH)] if $\mathscr L$ contains a tree language  $L \subseteq \trees \Sigma$, $\Gamma$ is a signature, and
		\begin{align*}
			\alpha: \clo \Gamma \to \clo \Sigma
		\end{align*}
		is a clone morphism, then $\mathscr L$ also contains $\alpha^{-1}(L)$.
	\end{itemize}
	Then if a language belongs to $\mathscr L$, then every language recognised by its syntactic clone also belongs to $\mathscr L$.
% A language belongs to $\mathscr L$ if and only if it is recognised by a clone from $\clo \mathscr L$.
\end{lem}
\begin{proof}
By definition, if a language is recognised by a clone from $\clo \mathscr L$ then it belongs to $\mathscr L$. Let us prove the other implication. Suppose that $L \subseteq \trees \Sigma$ belongs to $\mathscr L$. We will show that the syntactic clone of $L$ belongs to $\clo \mathscr L$.  Let then $K$ be a language, over some signature $\Gamma$, which is recognised by a morphism 
\begin{align*}
		\beta : \clo \Gamma \to \Cc_L.
\end{align*}
Since the syntactic morphism is surjective, it follows that there is a clone morphism $\gamma$ which makes the following diagram commute.
\begin{align*}
	\vcenter{\xymatrix @R=1pc { \clo \Sigma  \ar[r]^{\alpha_L} & \Cc_L  \\
	\clo \Gamma \ar[u]_\gamma \ar[ur]_\beta
	}}
\end{align*}
In particular, every language recognised by the morphism $\beta$ is an inverse image, under $\gamma$, of some language recognised by the syntactic morphism  $\alpha_L$. Therefore, by closure of $\mathscr L$ under inverse images of clone morphisms, it suffices to show that every language recognised by $\alpha_L$ belongs to $L$.  Since every language recognised by the syntacic morphism of $L$ is a finite union of equivalence classes of $L$-equivalence, we will be done if we show the following claim.
\begin{lem}
		Let $L$ be a regular tree language.  For every tree $t$, the set of trees that are $L$-equivalent to $t$ is a finite Boolean combination of quotients of $L$. 
	\end{lem}
	\begin{proof}
		By definition, a tree $s$ is $L$-equivalent to $t$ if and only if 
		\begin{align*}
			ps \in L \qquad \mbox{iff} \qquad pt \in L \qquad \mbox{holds for every $p \in \polar 1 \Sigma$}.
		\end{align*}
	If $p,q \in \polar 1 \Sigma$ have the same image under the syntactic clone morphism, then
		\begin{align*}
			ps \in L \qquad \mbox{iff} \qquad qs \in L \qquad \mbox{holds for every $s \in \trees \Sigma$}
		\end{align*}
		By regularity of $L$, one can choose a finite set $P \subseteq \polar 1 \Sigma$, such that $P$ and $\polar 1 \Sigma$ have the same image under the syntactic clone morphism of $L$. It follows that a tree $s$ is $L$-equivalent to $t$ if and only if 
		\begin{align*}
			ps \in L \qquad \mbox{iff} \qquad pt \in L \qquad \mbox{holds for every $p \in P$}.
		\end{align*}
		The set of trees $s$ which satisfy the condition above is easily seen to be a finite Boolean combination of quotients of $L$. % namely
 % 		\begin{align*}
 % 			\bigcap_{p \in P : pt \in L} p^{-1} L  \qquad - \qquad \bigcup_{p \in P : pt \not \in L}  p^{-1}L.
 % 		\end{align*}
	\end{proof}
 
\end{proof}

A class of regular languages satisfying assumptions (LQ), (LB) and (LH) in the above lemma is called a \emph{clone variety of languages}. As shown in Example~\ref{ex:potthof}, the class of first-order definable tree languages does not satisfy the conclusions of the above lemma, and therefore it is not a clone variety of languages. As shown in the following example, the problem is with (LH).


\begin{ourexample}\label{ex:fo-not-variety}
The class of first-order definable tree languages satisfies conditions (LQ) and (LB) in Lemma~\ref{lem:clone-invariant}, but fails condition (LH), about inverse images of clone morhpisms. The issue is that a clone morhpism can duplicate trees. For instance, let $f_0,f_1,f_2$ be letters as in the previous example, of arities $0,1,2$ respectively. Consider the signatures $\Sigma = \set{f_0,f_2}$ and $\Gamma=\set{f_0,f_1}$. As discussed in the previous example, the set of trees where every leaf is at even depth is first-order definable when the signature is $\Sigma$, but is not first-order definable when the signature is $\Gamma$ (note that in the latter case every tree has just one leaf).  Consider the morphism 
\begin{align*}
	\alpha : \clo \Gamma \to \clo \Sigma
\end{align*}
which maps $f_0$ to $f_0$, and which maps $f_1(t)$ to $f_2(\alpha(t),\alpha(t))$. This morphism maps a tree that looks like a line to a complete binary tree of the same depth. The set of trees over $\Gamma$ which have the unique leaf at even depth is the inverse image under $\alpha$ of the set of trees over $\Gamma$ which have every at even depth. One can show that the first-order definable tree languages satisfy a weak condition than (LH), where morphisms are restricted to nonduplicating ones, i.e.~morphisms $\alpha$ where a tree $a(t_1,\ldots,t_n)$ is mapped to a term which uses each of  $\alpha(t_1),\ldots,\alpha(t_n)$ at most once.
\end{ourexample}


In Section~\ref{sec:varities}, we will that the class of tree languages definable in chain logic, as well as several other logics, form clone varities.


%
%


\subsection{An Eilenberg theorem.} 
In this section, we present clone version of the pseudovariety theorem of Eilenberg. The original theorem of Eilenberg~\cite{eilenberg1974automata} says that there is a one-to-one correspondence between classes of regular word languages satisfying certain closure properties, and classes of finite monoids satisfying certain closure properties.  In our clone version, Theorem~\ref{thm:eilenberg}, the classes of languages will be classes  of regular tree languages satisfying the assumptions in Lemma~\ref{lem:clone-invariant}, while the classes of clones will need to contain only finitely generated finite clones, and be closed under products, subclones, restricting the universe, and images under clone morphisms.
\paragraph*{Operations on  clones.}  A \emph{subclone} of $\Cc$ is obtained by removing some operations in $\Cc$. A \emph{restriction} (todo: find the correct word) is obtained from $\Cc$ by restricting the universe to a subset closed under all operations. A \emph{product} of two clones $\Cc$ and $\Dd$ has the product of their universes as the universe, and has an operation
\begin{align*}
	((c_1,d_1),\ldots,(c_n,d_n)) \qquad \mapsto \qquad (f(c_1,\ldots,c_n),g(d_1,\ldots,d_n)
\end{align*}
for every $n$-ary operations $f$ and $g$ in $\Cc$ and $\Dd$ respectively.

\paragraph*{Finitely generated clones.} A clone is called \emph{finitely generated} if it is generated by an algebra with a finite set of fundamental operations. Finitely generated clones are closed under restrictions and products, but not under subclones, as shown in the following example. 

\begin{ourexample}\label{ex:yakov-muchnik}
The clone of all operations on the universe $\set{1,2,3}$ is finitely generated, e.g.~by the three constants $1$,  $2$, and $3$ and the operation
\begin{align*}
	\mathtt{ifthenelse}(a,b,c,d) = \begin{cases}
		c & \mbox{if $a=b$}\\
		d & \mbox{ otherwise}.
	\end{cases}
\end{align*}
Therefore every clone on this universe is a subclone of a finitely generated clone. As shown by Muchnik and Yanov in~\cite{yanovmuchnik}, there exist clones over this universe which are not finitely generated. \end{ourexample}

\paragraph*{From classes of clones to classes of languages and back.}
 If $\mathscr L$ is a class of regular languages, then define $\clo \mathscr L$ to be the class of all  finitely generated clones $\Cc$ with finite universe such that every tree language recognised by $\Cc$ belongs to $\mathscr L$.  Conversely, if $\mathscr C$ is a class of finite clones, then define $\lang \mathscr L$ to be the class of languages recognised by clones from $\mathscr C$.
 
 We are now ready to state the Eilenberg theorem.
 \begin{thm}\label{thm:eilenberg}
 	The mappings $\mathscr L \mapsto \clo \mathscr L$ and $\mathscr C \mapsto \lang {\mathscr C}$ are mutually inverse bijections between: 
	\begin{enumerate}
		\item[(L)] \label{it:lang-pseudovariety} classes of languages satisfying conditions (LQ), (LB) and (LH) in Lemma~\ref{lem:clone-invariant};
		\item[(C)] \label{it:clone-pseudovariety} classes of finitely generated clones closed under finitely generated subclones, restrictions, products, and images of clone morphisms.
	\end{enumerate}
 \end{thm}
 \begin{proof}
	 We first show that $\mathscr L \mapsto \clo \mathscr L$  takes classes as in item~\ref{it:lang-pseudovariety} to classes as in~\ref{it:clone-pseudovariety}, while the mapping $\mathscr C \mapsto \lang {\mathscr C}$ goes the other way.  
	 Actually, $\mathscr C \mapsto \lang {\mathscr C}$ maps every class of clones closed under products to a class of languages as in (L), while $\mathscr L \mapsto \clo \mathscr L$ maps every class of languages closed under Boolean operations to a class of clones as in (C).
	
	The less obvious part, and the one where all the closure properties are used, is that the two mappings are mutually inverse. We first show that 
	\begin{align*}
		\mathscr L  = \lang (\clo \mathscr L) \qquad \mbox{if $\mathscr L$ is a class of  languages as in (L).}
	\end{align*}
	A language $L$  belongs to the right side of the equality if it is recognised by some clone $\Cc$, such that every language recognised by $\Cc$ belongs to $\mathscr L$.  Therefore, the inclusion $\supseteq$ is immediate.  For the opposite inclusion, suppose that $L$  belongs to $\Ll$. By Lemma~\ref{lem:clone-invariant}, the syntactic clone of $L$ belongs to $\clo \mathscr L$, and therefore $L$ belongs to the right side.
	

	
To complete the proof of the theorem, it remains to show that
	\begin{align*}
		\mathscr C  = \clo (\lang \mathscr C) \qquad \mbox{if $\mathscr C$ is a  class of clones as in (C).}
	\end{align*}
	A clone $\Cc$ belongs to the right side of the equality if every language recognised by it is recognised by some clone in $\mathscr C$. Therefore, the inclusion $\subseteq$ is immediate.  For the converse inclusion, suppose that $\Cc$ belongs to the right side.  By definition of the mapping $\mathscr L \mapsto \clo \mathscr L$, the clone $\Cc$ is finitely generated. Let $C$ be the universe of the clone, and let $\Sigma$ be the family of operations which generate it. This family can be viewed as a signature, and therefore there exists a surjective morphism
	\begin{align*}
		\alpha : \clo \Sigma \to \Cc.
	\end{align*}
For every $c \in C$, define $L_c \subseteq \trees \Sigma$ to be the set of terms that evaluate to $c$. By the assumption that $\Cc$ belongs to $\clo (\lang \mathscr C)$, each language $L_c$ is recognised by some morphism
	\begin{align*}
		\beta_c : \clo \Sigma \to \Dd_c \qquad \mbox{with $\Dd_c \in \mathscr C$}.
	\end{align*}
	Let $\beta$ be the product of all these morphisms, and let its image be $\Dd$. Note that  $\Dd$ belongs to $\mathscr C$, because it  is a finitely generated subclone of a product of clones from $\mathscr C$. Summing up, we have the  following diagram 
	\begin{align*}
		\vcenter{\xymatrix @R=1pc { \clo \Sigma  \ar[r]^{\beta} \ar[d]^{\alpha} & \Dd  \\
		\Cc
		}}
	\end{align*}
	where both $\alpha$ and $\beta$ are surjective. The mapping $\beta$ recognises all of the languages $L_c$, and therefore (todo: check this therefore) the kernel of $\alpha$ is coarser than the kernel of $\beta$. This implies that there is a clone morphism from $\Dd$ to $\Cc$ which makes the diagram commute, and therefore $\Cc$ belongs to $\mathscr C$ by virtue of being an image of a clone from $\mathscr C$.
 \end{proof}
 


==> varieties.tex <==
\section{Classes of languages that are clone varieties} 
\label{sec:varities}
As  shown in Example~\ref{ex:potthof}, the first-order definable tree languages do not form a clone variety of languages. In this section we show several examples of classes of languages that do form clone varieties.



\subsection{Path languages} 

\paragraph*{Path language.} For a signature $\Sigma$, define $[\Sigma]$ to be the set  of all pairs $(a,i)$ such that $a$ is an $n$-ary symbol in $\Sigma$ and $i \in \set{1,\ldots,n}$. We will treat $[\Sigma] \cup \Sigma$ as an alphabet for words. For a path  $\pi$ in a tree  $t \in \trees \Sigma$, define its \emph{labelling}, denoted by $[\pi]_t$, to be the word in $[\Sigma]^* \Sigma$  whose definition is illustrated in the following picture:
\begin{center}
	(TODO: draw the picture)
\end{center}
For a word language $L \subseteq [\Sigma]^*\Sigma$, define  $\mathsf A L$ to be the set of trees $t \in \trees \Sigma$ such that the labelling of every root-to-leaf path belongs to $L$. A language of the form $\mathsf A L$ for $L$ a regular word language is called a \emph{universal path language}.  Universal path languages are exactly the tree languages recognised by deterministic root-to-leaves automata as defined in~\cite{}. A tree language $L$ is universal if and only if it is equal to
\begin{align*}
	\mathsf A \set{[\pi]_t : \mbox{$\pi$ is a root-to-leaf path in some $t \in L$}},
\end{align*}
in particular one can decide -- using an equality check on tree automata -- if a tree language is universal.  



Let $\boolpi 1$ be the set of trees that represent a Boolean formula that only uses $\land,0,1$ and which has value $1$.  This is a special case of languages   $\boolpi n$ and $\boolsigma n$, with $n \in \Nat$, which will be defined and studied later on. An easy check shows the following lemma.
\begin{lemma}\label{lem:universal-reduces}
	(a) A language is a universal path language if and only if it reduces to the language $\boolpi 1$. (b) A language or its complement is a universal path language  if and only if it reduces to a language recognised by the semilattice.
\end{lemma}


Universal path languages are not closed under intersection but not under union or  complement.
A \emph{path language} is defined to be a finite Boolean combination of universal path languages.  It is not known (maybe it will be once this paper is written:) if one can decide whether or not a tree language is a path language.

\paragraph*{Path clones.} Let $M$ be a finite monoid. The \emph{path clone of $M$}, denoted by  $\pathclone M$, is defined to be the clone where the universe is the powerset of $M$, and for every $m_1,\ldots,m_n \in M$ there is an $n$-ary operation
\begin{align}
	\label{eq:definition-of-a-path-clone}
		M_1,\ldots,M_n \subseteq M \qquad \mapsto \qquad m_1 M_1 \cup \cdots \cup m_n M_n.
\end{align}

% \paragraph*{Path algebras.} Let $(Q,S)$ be a transformation semigroup. The \emph{path algebra} associated to this transformation group is defined as follows. The universe is $P(Q)$. There is a constant for every singleton. For every $s_1,\ldots,s_n \in S$, there is an $n$-ary operation defined by
% \begin{align*}
% 	Q_1,\ldots,Q_n \qquad \mapsto \qquad \bigcup Q_i s_i,
% \end{align*}
% where $Q_i s_i$ stands for the image of $Q_i$ under the action of $s_i$. A \emph{path clone} is a clone generated by a path algebra.


\begin{lemma}\label{lem:path-algebra-path-clone} The following conditions are equivalent for a tree language:
	\begin{enumerate}
		\item $L$ is a path language;
		\item $L$ is recognised by a path clone;
		\item $L$ is recognised by a matrix power of the semilattice $(\set{0,1},\land)$.
	\end{enumerate}Furthermore, path languages form a clone variety of tree languages.
\end{lemma}
\begin{pr}
Adjusting for a  different nomenclature, equivalence of items 1 and 2   is Lemma 2.4.8 in~\cite{doktorat-bojanczyk}. Equivalence of 1 and 3, follows from Lemmas~\ref{lem:universal-reduces} and~\ref{lem:reductions-vs-matrix}.
  Since the class of clones in item 3 is closed under products, it follows that  path languages form a clone variety.
\end{pr}

McKenzie shows in~\cite{} that one can decide if an algebra is a subalgebra of a path algebra, which implies that one can decide if a finitely generated clone is a sobclone of a path clone.
Unfortunately, this result is not sufficient to decide if a regular language is a path language, because the syntactic algebra of a path language is in general a morphic image of a subclone of a path clone. (todo: check that the claims in this paragraph are correct). 

\begin{ourexample}
	This example shows that a path clone can have uncountably many subclones. Consider a monoid $M$. Recall that there is a one-to-one correspondence between finite sequences over $M$ and operations in $\pathclone M$. Furthermore, for every subclone of $\pathclone M$, if it contains an operation corresponding to a sequence, then the subclone also contains an operation corresponding to any 
	
	For a family $X$ of finite multisets over $M$, define $\pathclone X$ to be the smallest family that contains $X$, and such that if  $\pathclone X$ contains multisets $A,B$, then for every element $m \in A$, the family $\pathclone X$ contains the multiset obtained from $A$ by removing one copy of $m$, and adding the multiset $m \cdot B$.	%
	% \begin{align*}
	% 	\set{m_1,\ldots,m_k} \qquad \set{n_1,\ldots,n_l}
	% \end{align*}
	% then it also contains the multiset
	% \begin{align*}
	% 	\set{m_2,\ldots,m_k} \cup \set{m_1 n_1,\ldots,m_1 n_l}.
	% \end{align*}
	One can show that for every multiset $X$, the set of operations
	\begin{align*}
			M_1,\ldots,M_n \subseteq M \qquad \mapsto \qquad m_1 M_1 \cup \cdots \cup m_n M_n.
	\end{align*}
	such that $\set{m_1,\ldots,m_n}$ is a multiset in $\pathclone X$, is a subclone of $\pathclone M$. In fact, every subclone is of this form.
	
	Let $M$ be the group  $\Int_3 \times \Int_3$. Consider
	\begin{align*}
		a = (0,1) \qquad b=(1,0),
	\end{align*}
	and let $Y$ be the infinite family of multisets which contain at least one $a$, at least one $b$, and no other elements of $M$. One can show that 
	\begin{align*}
		\pathclone X \cap Y = X \qquad \mbox{for every $X \subseteq Y$}.
	\end{align*}
	Since $X$ can be chosen in an uncountable number of ways, it follows that $\pathclone M$ has uncountably many subclones.
\end{ourexample}

\subsection{Chain logic} Recall that chain logic is the fragment of monadic second-order logic where set quantification is restricted to chains.

\begin{lemma}\label{lem:algebraic-chain-logic}
	The following conditions are equivalent for a tree language $L$:
\begin{enumerate}
	\item $L$ is definable in chain logic;
	\item $L$ is recognised by a wreath product of  path algebras.
		\item $L$ is recognised by a wreath product of  matrix powers of $(\set{0,1},\land)$.
\end{enumerate}
Furthermore, the class of language definable in chain logic is a clone variety.
\end{lemma}
\begin{pr}
Adjusting for a  different nomenclature, the equivalence of 1 and 2 is Theorem 2.5.9 in~\cite{doktorat-bojanczyk}. Equivalence of items 2 and 3 follows from Lemma~\ref{lem:path-algebra-path-clone}. Since the clones in item 3 are closed under products, it follows that chain logic is a clone variety.
\end{pr}




\subsection{CTL} The syntax and semantics of \emph{computation tree logic,}  \ctl for short, over finite trees over a ranked alphabet $\Sigma$ is defined as follows.
\begin{itemize}
	\item If $a$ is a letter in $\Sigma$, then $a$ is a formula of \ctl, which is true in trees that have $a$ in the root;
	\item Boolean combinations are allowed, with the usual semantics;
	\item If $\varphi$ is a formula of \ctl, and $i$ is a natural number, then $\mathsf X_i \varphi$ is a formula of \ctl. This formula is true in a tree $t$ if the root has an $i$-th child, and the subtree rooted in the $i$-th child  satisfies $\varphi$.	
	\item If $\varphi$ and $\psi$ are formulas of \ctl, then $\mathsf E \varphi \mathsf U \psi$ is a formula of \ctl. This formula is true in a tree $t$ if there exists a node $v$ of $t$ such that $\psi$ is true in the subtree $t|_v$, and  $\varphi$ is true in   $t|_w$ for every node $w$ on the path from the root to $v$, not including the root nor $v$.
\end{itemize}
The logic \ctl is one of the natural tree generalisations of \ltl. Recall that \ltl is a temporal logic, which for words (both finite and infinite) has the same expressive power as first-order logic. Another natural tree generalisation of \ltl is {\sc ctl*}, which in one formalisation has the same expressive power as first-order logic, see~\cite{haferthomas}, and therefore need not be separately discussed here. 

The logic \ctl is easily seen to be expressively equivalent to a fragment of first-order logic, this fragment is strict as shown in the following example.
\begin{ourexample}
	Let the signature consist of one constant $c$, and two binary symbols $a,b$.  The language is those trees where for some root-to-leaf path, the sequence of labels is in $(ab)^*c$. This language is definable in first-order logic, but not in \ctl.
\end{ourexample}


\begin{lemma}\label{lem:wreath-characterisation-of-ctl}
	The following conditions are equivalent for a tree language:
		\begin{enumerate}
			\item $L$ is definable in \ctl;
			\item $L$ is recognised by a wreath power of the semilattice $(\set{0,1},\land)$.
		\end{enumerate}Furthermore, languages definable in \ctl form a clone variety of tree languages.
\end{lemma}
\begin{pr}
	Adjusting for a  different nomenclature, the equivalence of 1 and 2 is proved in (dac wlasciwy link typu Ivan, czy Ivan Esik). Since the clones in item 2 are closed under products, it follows that tree languages definable in \ctl form a clone variety.
\end{pr}



